Enhanced Performance of Pre-Trained Networks by Matched Augmentation Distributions

There exists a distribution discrepancy between training and testing, in the way images are fed to modern CNNs. Recent work tried to bridge this gap either by fine-tuning or re-training the network at different resolutions. However re-training a network is rarely cheap and not always viable. To this end, we propose a simple solution to address the train-test distributional shift and enhance the performance of pre-trained models -- which commonly ship as a package with deep learning platforms \eg, PyTorch. Specifically, we demonstrate that running inference on the center crop of an image is not always the best as important discriminatory information may be cropped-off. Instead we propose to combine results for multiple random crops for a test image. This not only matches the train time augmentation but also provides the full coverage of the input image. We explore combining representation of random crops through averaging at different levels \ie, deep feature level, logit level, and softmax level. We demonstrate that, for various families of modern deep networks, such averaging results in better validation accuracy compared to using a single central crop per image. The softmax averaging results in the best performance for various pre-trained networks without requiring any re-training or fine-tuning whatsoever. On modern GPUs with batch processing, the paper's approach to inference of pre-trained networks, is essentially free as all images in a batch can all be processed at once.

==> extras.tex <==
\begin{table*}[ht]
\centering
\caption{
Comparison of \textbf{Top-1} validation accuracy on ImageNet dataset for ResNet \cite{He2016Deep} family. 
The performance gain in each case is noted in parentheses. 
$^\dagger$ indicates the numbers reported on the PyTorch page \cite{pytorch} and verified on our end. Whereas $^\ddagger$ indicates the numbers taken from \cite{Yun2019CutMix}. 
It should be noted that the numbers reported for baseline ResNets in \cite{Yun2019CutMix} are higher than PyTorch and have been noted below, so the improvement is with respect to those baseline and not of PyTorch.
The numbers reported for all other approaches are taken from their respective papers. 
For consistent comparison we report the accuracy for all approaches where train and test resolution is fixed to $224\times224$ and specifically note the variants where test resolution deviates.
Averaging  the softmax (SM) scores of random crops (RCs) results in better performance than that of averaging at the deep feature vector (FV) level. 
The performance gain is high for smaller networks and low for larger ones. 
An increase in the number of crops results in enhanced performance, however, performance gain saturates after a certain number of crops as evidenced in Fig \ref{fig_resnet_performance}.
}
\resizebox{0.98\textwidth}{!}{
\label{table_resnet}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Approach & Custom Training & ResNet-18 & ResNet-34 & ResNet-50 & ResNet-101 & ResNet-152\\ \hline
Feature Dimension & - & 512 & 512 & 2048 & 2048 & 2048\\
Image Resized To & - & 256 & 256 & 256 & 256 & 256\\
Input Crop Size & - & $224\times224$ & $224\times224$ & $224\times224$ & $224\times224$ & $224\times224$\\
Crop to Image Ratio & - & 0.875 & 0.875 & 0.875 & 0.875 & 0.875\\ \hline

Center Crop$^\dagger$ & - & 69.76 & 73.31 &	76.13 & 77.37 & 78.31 \\ \hline
\textbf{Ours} \scriptsize(Average of FV of 10 RCs) & \textcolor{darkergreen}{\xmark} & $71.42^{\textbf{(+1.66)}}$ & $74.74^{\textbf{(+1.43)}}$ & $77.22^{\textbf{(+1.09)}}$ & $78.46^{\textbf{(+1.09)}}$ & $79.39^{\textbf{(+1.08)}}$ \\ 
\textbf{Ours} \scriptsize(Average of FV of 20 RCs) & \textcolor{darkergreen}{\xmark} & $71.56^{\textbf{(+1.80)}}$ & $74.93^{\textbf{(+1.62)}}$ & $77.30^{\textbf{(+1.17)}}$ & $78.65^{\textbf{(+1.28)}}$ & $79.54^{\textbf{(+1.23)}}$ \\
\textbf{Ours} \scriptsize(Average of SM of 10 RCs) & \textcolor{darkergreen}{\xmark} & $71.64^{\textbf{(+1.88)}}$ & $74.88^{\textbf{(+1.57)}}$ & $77.44^{\textbf{(+1.31)}}$ & $78.67^{\textbf{(+1.30)}}$ & $79.58^{\textbf{(+1.27)}}$ \\ 
\textbf{Ours} \scriptsize(Average of SM of 20 RCs) & \textcolor{darkergreen}{\xmark} & $71.83^{\textbf{(+2.07)}}$ & $75.14^{\textbf{(+1.83)}}$ & $77.49^{\textbf{(+1.36)}}$ & $78.85^{\textbf{(+1.48)}}$ & $79.79^{\textbf{(+1.48)}}$ \\ \hline
MEAL \cite{Shen2019MEAL}                        &       \textcolor{red2}{\cmark} & - & - & 76.42 & - & - \\ 
MEAL Plus \cite{Shen2019MEAL}                   &       \textcolor{red2}{\cmark} & - & - & 78.21 & - & - \\
MEAL V2 \cite{Shen2021MEAL}                     &       \textcolor{red2}{\cmark} & 73.19 & - & 80.67 & - & - \\ \hline
Baseline$^\ddagger$                             &       - & - & - & 76.32 & 78.13 & - \\
Cutout$^\ddagger$ \cite{DeVries2017Improved}    &       \textcolor{red2}{\cmark} & - & - & 77.07 & 79.28 & - \\
Mixup$^\ddagger$ \cite{Zhang2018mixup}          &       \textcolor{red2}{\cmark} & - & - & 77.42 & 79.48 & - \\
Manifold Mixup$^\ddagger$ \cite{Verma2019Manifold} &       \textcolor{red2}{\cmark} & - & - & 77.50 & - & - \\
CutMix$^\ddagger$ \cite{Yun2019CutMix}          &       \textcolor{red2}{\cmark} & - & - & 78.60 & 79.83 & - \\\hline
FixRes \cite{Touvron2019Fixing}                 &       \textcolor{red2}{\cmark} & - & - & 77.0 & - & - \\ 
FixRes \cite{Touvron2019Fixing} \scriptsize$(\text{adaptation + augmentation})$   &       \textcolor{red2}{\cmark} & - & - & 77.1 & - & - \\
FixRes \cite{Touvron2019Fixing} \scriptsize$(\text{adaptation + augmentation + @ 384})$   &       \textcolor{red2}{\cmark} & - & - & 79.1 & - & - \\
FixRes \cite{Touvron2019Fixing} \scriptsize$(\text{adaptation + augmentation + @ 320 + Billion-scale})$   &       \textcolor{red2}{\cmark} & - & - & 82.5 & - & - \\
\end{tabular}
}
\vspace{-0.05in}
\end{table*}

